Convergence properties of optimal transport-based temporal networks

We study network properties of networks evolving in time based on optimal transport principles. These evolve from a structure covering uniformly a continuous space towards an optimal design in terms of optimal transport theory. At convergence, the networks should optimize the way resources are transported through it. As the network structure shapes in time towards optimality, its topological properties also change with it. The question is how do these change as we reach optimality. We study the behavior of various network properties on a number of network sequences evolving towards optimal design and find that the transport cost function converges earlier than network properties and that these monotonically decrease. This suggests a mechanism for designing optimal networks by compressing dense structures. We find a similar behavior in networks extracted from real images of the networks designed by the body shape of a slime mold evolving in time.

==> preamble/preamble_usepackage.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our additions of packages: 
\usepackage[english]{babel}


\usepackage{amsmath,fixmath}
%\usepackage{comment}
\usepackage{lineno}
\usepackage[explicit]{titlesec}

% FIGURES
%\usepackage[caption=false]{subfig}
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% TABLES
\usepackage{tabularx}
%\usepackage{booktabs}
\usepackage[justification=justified, format=plain]{caption}

% ALGORITHMS
\usepackage{algorithm,algorithmic}

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

\hypersetup{
 bookmarks=true, % show bookmarks bar?
 unicode=false, % non-Latin characters in Acrobat�s bookmarks
 pdftoolbar=true, % show Acrobat�s toolbar?
 pdfmenubar=true, % show Acrobat�s menu?
 pdffitwindow=false, % window fit to page when opened
 pdfstartview={FitH}, % fits the width of the page to the window
 pdftitle={}, % title
 pdfauthor={}, % author
 pdfcreator={}, % creator of the document
 pdfproducer={}, % producer of the document
 pdfkeywords={} {} {}, % list of keywords
 pdfnewwindow=true, % links in new window
 colorlinks=true, % false: boxed links; true: colored links
 linkcolor=red, % color of internal links
 filecolor=magenta, % color of file links
 urlcolor=cyan % color of external links
  %citecolor=ForestGreen, % color of links to bibliography
}
